On the Feasibility of In-Context Probing for Data Attribution

Data attribution methods are used to measure the contribution of training data towards model outputs, and have several important applications in areas such as dataset curation and model interpretability. However, many standard data attribution methods, such as influence functions, utilize model gradients and are computationally expensive. In our paper, we show in-context probing (ICP) -- prompting a LLM -- can serve as a fast proxy for gradient-based data attribution for data selection under conditions contingent on data similarity. We study this connection empirically on standard NLP tasks, and show that ICP and gradient-based data attribution are well-correlated in identifying influential training data for tasks that share similar task type and content as the training data. Additionally, fine-tuning models on influential data selected by both methods achieves comparable downstream performance, further emphasizing their similarities. We also examine the connection between ICP and gradient-based data attribution using synthetic data on linear regression tasks. Our synthetic data experiments show similar results with those from NLP tasks, suggesting that this connection can be isolated in simpler settings, which offers a pathway to bridging their differences.

==> figures/bertscore-icp-infl.tex <==
\begin{figure*}[h!]
  \centering 
  \begin{subfigure}{0.6\linewidth}
    \includegraphics[width=\linewidth]{images/bertscore_icp_infl.png}
  \end{subfigure}
  \caption{Bertscore vs. Spearman Correlation between ICP and $\text{Infl}_{\text{IP}}$ for instruction data}
  \label{fig:bertscore-icp-infl}
\end{figure*}

==> figures/content-similiarity-new.tex <==
\begin{figure*}[t!]
    \subfloat[test]{
        {\includegraphics[width=0.24\linewidth]{images/nlp_exp_images/bertscore_alpaca_alpaca_llama.png}}
        \label{fig:content-similarity-alpaca-llama}
        }
    \subfloat[test]{
        {\includegraphics[width=0.24\linewidth]{images/nlp_exp_images/bertscore_alpaca_alpaca_pythia.png}}
        \label{fig:content-similarity-alpaca}
        }
    \subfloat[test]{
        {\includegraphics[width=0.24\linewidth]{images/nlp_exp_images/bertscore_qa_qa_pythia.png}}
        \label{fig:content-similarity-qa}
        }
    \subfloat[test]{
        {\includegraphics[width=0.24\linewidth]{images/nlp_exp_images/bertscore_docqa_docqa_pythia.png}}
        \label{fig:content-similarity-docqa}
        }
    %\vspace{-1.8\baselineskip}
    \caption{Correlation analysis between ICP, $\text{Infl}_{\text{Loc}}$, and $\text{Infl}_{\text{IP}}$ with respect to content similarity (BertScore) using test and train samples from the same task.}
    \label{fig:content-similarity}
\end{figure*}

\begin{comment}
\begin{subfigure}{0.24\linewidth}
    \includegraphics[width=\linewidth]{images/nlp_exp_images/bertscore_alpaca_alpaca_llama.png}
    \label{fig:content-similarity-alpaca-llama}
    \caption{test}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
    \includegraphics[width=\linewidth]{images/nlp_exp_images/bertscore_alpaca_alpaca_pythia.png}
    \label{fig:content-similarity-alpaca}
    \caption{test}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
    \includegraphics[width=\linewidth]{images/nlp_exp_images/bertscore_qa_qa_pythia.png}
    \label{fig:content-similarity-qa}
    \caption{test}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
    \includegraphics[width=\linewidth]{images/nlp_exp_images/bertscore_docqa_docqa_pythia.png}
    \label{fig:content-similarity-docqa}
    \caption{test}
  \end{subfigure}
\end{comment}

==> figures/lin-func-heatmaps-change.tex <==
\begin{figure*}[h!]
  \centering 
  \nocaption
  \begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_task_input_n1_change_loss.png}
    \caption{$k=1$}
    \label{fig:lin-func-task-input-n1-change-loss} 
  \end{subfigure}
  \begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_task_input_n5_change_loss.png}
    \caption{$k=5$}
    \label{fig:lin-func-task-input-n5-change-loss} 
  \end{subfigure}
  \begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_task_input_n10_change_loss.png}
    \caption{$k=10$}
    \label{fig:lin-func-task-input-n10-change-loss} 
  \end{subfigure}
  \begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_task_input_n20_change_loss.png}
    \caption{$k=20$}
    \label{fig:lin-func-task-input-n20-change-loss} 
  \end{subfigure}
  \begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_task_input_n40_change_loss.png}
    \caption{$k=40$}
    \label{fig:lin-func-task-input-n40-change-loss} 
  \end{subfigure}
  \caption{Change in output loss as \textit{both} against the baseline test query as content and task similarity of the ICL training demonstrations vary with respect to the test query ($k$ denotes the number of in-context demonstrations in the prompt sequence).}
  \label{fig:lin-func-heatmap-change}
\end{figure*}

==> figures/lin-func-heatmaps.tex <==
\begin{figure*}[h!]
  \centering 
  \nocaption
  \begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_task_input_n1_loss.png}
    \caption{k=1}
  \end{subfigure}
  \begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_task_input_n5_loss.png}
    \caption{k=5}
  \end{subfigure}
  \begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_task_input_n10_loss.png}
    \caption{k=10}
  \end{subfigure}
  \begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_task_input_n20_loss.png}
    \caption{k=20}
  \end{subfigure}
  \begin{subfigure}{0.32\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_task_input_n40_loss.png}
     \caption{k=40}
  \end{subfigure}
  \caption{Output loss as \textit{both} against the baseline test query as content and task similarity of the ICL training demonstrations vary with respect to the test query ($k$ denotes the number of in-context demonstrations in the prompt sequence).}
  \label{fig:lin-func-heatmap}
\end{figure*}

==> figures/lin-func-input-task-loss.tex <==
\begin{figure}
  \nocaption
  \begin{subfigure}{0.35\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_input_loss.png}
    \caption{Content}
    \label{fig:lin-func-input-loss} 
  \end{subfigure}
  \begin{subfigure}{0.35\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_task_loss.png}
    \caption{Task}
    \label{fig:lin-func-task-loss} 
  \end{subfigure}
  \begin{subfigure}{0.2\linewidth}
    \includegraphics[width=\linewidth]{images/lin_func_images/lin_func_legend.png}
    \vspace{0.7\linewidth}
  \end{subfigure}
  \caption{Squared error as the content and task similarity of the ICL training demonstrations vary with respect to the test query.}
  \label{fig:lin-func-input-task}
\end{figure}

==> sections/temporary_theory_notes.tex <==
\section{Theory (notes)}

Prior literature has suggested that in-context learning may implicitly perform gradient descent. For example, \citet{vonoswald2023} hypothesizes that transformers trained to perform linear regression in-context by gradient descent, by implicitly descending the function \begin{align}
    X
\end{align}

==> tables/bertscore.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{ccc}
        \toprule 
        & BertScore Top x &  BertScore Bottom x \\
        \midrule
        ICP/$\text{Infl}_{\text{IP}}$ & & \\
        ICP/One-Step & & \\
        One-Step/$\text{Infl}_{\text{IP}}$ & & \\
        \bottomrule
    \end{tabular}
    \caption{Avg. Spearman Correlation between ICP, One-Step, and $\text{Infl}_{\text{IP}}$ with respect to semantic (bertscore) similarity between train and test samples}
    \label{tab:bertscore}
\end{table}

==> tables/task-types.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{cccc}
        \toprule 
        & QA &  DocQA & Pretrain \\
        \midrule
        ICP/$\text{Infl}_{\text{IP}}$ & & &  \\
        ICP/One-Step & & \\
        One-Step/$\text{Infl}_{\text{IP}}$ & & &  \\
        \bottomrule
    \end{tabular}
    \caption{Spearman Correlation between ICP, One-Step, and $\text{Infl}_{\text{IP}}$ with respect task types}
    \label{tab:task-type}
\end{table}

==> tables/winrate-table.tex <==
\begin{table*}[t!]
\centering
\caption{Results (winrates) evaluated on the Alpaca Eval dataset after being finetuned on data selected by ICP and $\text{Infl}_\text{IP}$. The highest winrate in each column is marked with $*$ for ICP and $\dagger$ for $\text{Infl}_\text{IP}$.}
\scalebox{0.9}{
\begin{tabular}{l|r|lllllll}
    \toprule
    \textbf{Score Bin} & \textbf{Samples} & \textbf{Method} & \textbf{Helpful Base} & \textbf{Koala} & \textbf{Self Instruct} & \textbf{Oasst} & \textbf{Vicunna} & \textbf{Overall} \\
    \midrule
     $\leq 0.5$ & $4186$ & ICP & $47.65$ & $58.17$ & $59.2$ & $55.61$ & $61.25$ & $56.51$ \\
                & & $\text{Infl}_\text{IP}$  & $49.21$ & $57.79$ & $56.97$ & $59.89$ & $54.43$ & $56.31$ \\
     \hline
     $> 0.5$  & $47816$ & ICP & $57.03$ & $\mathbf{71.61^*}$ & $\mathbf{66.67^*}$ & $56.99$ & $61.53$ & $64.75$ \\
              &  & $\text{Infl}_\text{IP}$  & $54.33$ & $54.33$ & $\mathbf{66.67\dagger}$ & $54.33$ & $61.25$ & $58.88$ \\
     \hline
     $> 0.8$  & $20513$ & ICP & $\mathbf{66.41^*}$ & $69.07$ & $62.15$ & $\mathbf{67.57^*}$ & $63.75$ & $\mathbf{65.60^*}$ \\
              &  & $\text{Infl}_\text{IP}$  & $53.9$ & $\mathbf{70.39\dagger}$ & $63.2$ & $\mathbf{65.96\dagger}$ & $67.5$ & $\mathbf{64.17\dagger}$ \\
     \hline
     $> 0.85$ & $8012$ & ICP & $63.57$ & $67.94$ & $63.2$ & $63.98$ & $\mathbf{67.09^*}$ & $64.75$ \\
              &  & $\text{Infl}_\text{IP}$ & $\mathbf{61.42\dagger}$ & $68.18$ & $60.56$ & $63.83$ & $\mathbf{68.75\dagger}$ & $63.75$ \\
     \hline
     $> 0.9$ & $792$   & ICP & $46.51$ & $56.49$ & $52.77$ & $55.38$ & $56.96$ & $53.51$ \\
             &  & $\text{Infl}_\text{IP}$  & $53.91$ & $55.26$ & $54.58$ & $55.32$ & $48.75$ & $54.2$ \\
     \bottomrule
\end{tabular}
}
\label{tab:winrates}
\end{table*}
